GraphCloak: Safeguarding Task-specific Knowledge within Graph-structured Data from Unauthorized Exploitation

As Graph Neural Networks (GNNs) become increasingly prevalent in a variety of fields, from social network analysis to protein-protein interaction studies, growing concerns have emerged regarding the unauthorized utilization of personal data. Recent studies have shown that imperceptible poisoning attacks are an effective method of protecting image data from such misuse. However, the efficacy of this approach in the graph domain remains unexplored. To bridge this gap, this paper introduces GraphCloak to safeguard against the unauthorized usage of graph data. Compared with prior work, GraphCloak offers unique significant innovations: (1) graph-oriented, the perturbations are applied to both topological structures and descriptive features of the graph; (2) effective and stealthy, our cloaking method can bypass various inspections while causing a significant performance drop in GNNs trained on the cloaked graphs; and (3) stable across settings, our methods consistently perform effectively under a range of practical settings with limited knowledge. To address the intractable bi-level optimization problem, we propose two error-minimizing-based poisoning methods that target perturbations on the structural and feature space, along with a subgraph injection poisoning method. Our comprehensive evaluation of these methods underscores their effectiveness, stealthiness, and stability. We also delve into potential countermeasures and provide analytical justification for their effectiveness, paving the way for intriguing future research.

==> table/app/adv_more.tex <==

\begin{table}
\caption{Adv. training under budget 0.03}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccc} 
\toprule
\multirow{2}{*}{Models} & \multirow{2}{*}{Methods} & \multicolumn{4}{c}{Dataset}                 \\ 
\cmidrule{3-6}
                        &                          & MUTAG & ENZYMES & IMDB-BINARY & IMDB-MULTI  \\ 
\midrule
\multirow{6}{*}{GCN}    & Clean                    & 63.16 & 21.67   & 68.5        & 53.33       \\
                        & Random                   & 68.42 & 16.67   & 53.5        & 52.33       \\
                        & EMaxS                    & 68.42 & 16.67   & 58          & 51.33       \\
                        & EMinS                    & 36.84 & 16.67   & 55          & 56          \\
                        & EMinF                    & 65.79 & 16.67   & 67.5        & 44.33       \\
                        & SubInj                   & 65.79 & 14.17   & 55          & 41.17       \\ 
\midrule
\multirow{6}{*}{GIN}    & Clean                    & 89.47 & 15      & 51.5        & 33.33       \\
                        & Random                   & 78.95 & 20.83   & 49.5        & 33          \\
                        & EMaxS                    & 63.16 & 19.17   & 50          & 33.33       \\
                        & EMinS                    & 65.79 & 23.33   & 49          & 33.33       \\
                        & EMinF                    & 84.21 & 20      & 49.5        & 33.67       \\
                        & SubInj                   & 68.42 & 17.92   & 58.75       & 36.33       \\ 
\midrule
\multirow{6}{*}{Sage}   & Clean                    & 34.21 & 19.17   & 68.5        & 46          \\
                        & Random                   & 34.21 & 24.17   & 70          & 47.33       \\
                        & EMaxS                    & 34.21 & 23.33   & 66.5        & 34.33       \\
                        & EMinS                    & 57.89 & 23.33   & 67          & 41          \\
                        & EMinF                    & 76.32 & 22.5    & 64          & 40          \\
                        & SubInj                   & 76.32 & 22.08   & 52          & 30.67       \\
\bottomrule
\end{tabular}
}

\end{table}


==> table/medical-table.tex <==
\begin{table*}[t]
\caption{Case study for Medical datasets. 
% \rtodo{need more descriptions,like what's target and non-target? }
}
\label{tab:medcase_study}
\centering
% \renewcommand{\arraystretch}{0.9}
\resizebox{0.9\linewidth}{!}{
% \begin{tabular}{cccccccccccccc}
% \toprule
%  {\multirow{3}{*}{Models}} &
%    {\multirow{3}{*}{Methods}} &
%   \multicolumn{6}{c}{Tox21} &
%   \multicolumn{6}{c}{Odor} \\ \cline{3-14} 
%  {} &
%    {} &
%   \multicolumn{3}{c}{Targeted} &
%   \multicolumn{3}{c}{Non-targeted} &
%   \multicolumn{3}{c}{Targeted} &
%   \multicolumn{3}{c}{Non-targeted} \\ \cline{3-14} 
%  {} &
%    {} &
%    {before} &
%    {after} &
%    {drop} &
%    {before} &
%    {after} &
%    {drop} &
%    {before} &
%    {after} &
%    {drop} &
%    {before} &
%    {after} &
%   drop \\ \hline
% \multirow{3}{*}{GCN} &
%   EMinS &
%    {\multirow{3}{*}{76.00}} &
%    {67.00} &
%    {\textbf{9.00}} &
%    {\multirow{3}{*}{62.33}} &
%    {56.00} &
%   6.33 &
%    {\multirow{3}{*}{80.86}} &
%    {69.44} &
%    {\textbf{11.42}} &
%    {\multirow{3}{*}{72.84}} &
%    {65.97} & 6.87
%    \\ 
%  &
%    {EMinF} &
%    {} &
%    {60.33} &
%    {\textbf{15.67}} &
%    {} &
%    {52.67} &
%   9.66 &
%    {} &
%    {64.19} &
%    {\textbf{16.67}} &
%    {} &
%    {61.23} & 11.61
%    \\ 
%  &
%   SubInj &
%    {} &
%    {37.00} &
%    {\textbf{39.00}} &
%    {} &
%    {53.00} &
%   9.33 &
%    {} &
%    {44.44} &
%    {\textbf{36.42}} &
%    {} &
%    {63.28} & 9.56
%    \\ \hline 
% \multirow{3}{*}{GAT} &
%   EMinS &
%    {\multirow{3}{*}{76.33}} &
%    {72.33} &
%    {4.00} &
%    {\multirow{3}{*}{57.67}} &
%    {49.67} &
%    \textbf{8.00}&
%    {\multirow{3}{*}{76.54}} &
%    {57.58} &
%    {\textbf{18.96}} &
%    {\multirow{3}{*}{75.30}} &
%    {68.26} & 7.04
%    \\
%  &
%    {EMinF} &
%    {} &
%    {71.67} &
%    {\textbf{4.66}} &
%    {} &
%    {53.33} &
%    4.34&
%    {} &
%    {62.53} &
%    {\textbf{14.01}} &
%    {} &
%    {65.37} &  
%    {9.93} \\ 
%  &
%   SubInj &
%    {} &
%    {37.00} &
%    {\textbf{39.33}} &
%    {} &
%    {51.67} &
%    6.00&
%    {} &
%    {44.13} &
%    {\textbf{32.14}} &
%    {} &
%    {63.32} & 11.98
%    \\ \hline 
% \multirow{3}{*}{GIN} &
%   EMinS &
%    {\multirow{3}{*}{71.67}} &
%    {41.67} &
%    {\textbf{30.00}} &
%    {\multirow{3}{*}{59.00}} &
%    {53.00} &
%    6.00&
%    {\multirow{3}{*}{72.84}} &
%    {61.16} &
%    {\textbf{11.68}} &
%    {\multirow{3}{*}{71.60}} &
%    {62.93} & {8.67}
%    \\ 
%  &
%    {EMinF} &
%    {} &
%    {41.67} &
%    {\textbf{30.00}} &
%    {} &
%    {52.33} &
%    6.67&
%    {} &
%    {61.60} &
%    {\textbf{11.24}} &
%    {} &
%    {61.97} &
%    {9.63} \\
%  &
%   SubInj &
%    {} &
%    {36.67} &
%    {\textbf{35.00}} &
%    {} &
%    {51.67} &
%    7.33 &
%    {} &
%    {54.19} &
%    {\textbf{19.65}} &
%    {} &
%    {62.52} & 9.08
%    \\ \hline 
% \multirow{3}{*}{Sage} &
%   EMinS &
%    {\multirow{3}{*}{79.33}} &
%    {56.67} &
%    {\textbf{22.66}} &
%    {\multirow{3}{*}{65.33}} &
%    {56.33} &
%    9.00&
%    {\multirow{3}{*}{75.93}} &
%    {63.89} &
%    {\textbf{12.14}} &
%    {\multirow{3}{*}{73.14}} &
%    {64.52} & 8.62
%    \\
%  &
%    {EMinF} &
%    {} &
%    {65.33} &
%    {\textbf{14.00}} &
%    {} &
%    {56.00} &
%    9.33&
%    {} &
%    {64.13} &
%    {\textbf{11.80}} &
%    {} &
%    {63.09} &
%    {10.09} \\ 
%  &
%   SubInj &
%    {} &
%    {40.33} &
%    {\textbf{39.00}} &
%    {} &
%    {56.67} &
%    8.66&
%    {} &
%    {55.86} &
%    {\textbf{20.07}} &
%    {} &
%    {64.94} & 8.20
%    \\ 
%    \bottomrule
% \end{tabular}

\begin{tabular}{cc|ccc|ccc} 
\toprule
\multirow{3}{*}{Models} & \multirow{3}{*}{Methods} & \multicolumn{6}{c}{Tox21}                                                                        & \multicolumn{6}{c}{Odor}                                                                  \\ 
\cline{3-14}
                        &                          & \multicolumn{3}{c}{Targeted}                    &               & \multicolumn{3}{c}{Targeted}                           \\ 
\cline{3-14}
                        & & before & after & drop    & before  & after & drop              \\ 
\hline
\multirow{3}{*}{GCN}    & EMinS                    & \multirow{3}{*}{76.00} & 67.00 & \textbf{9.00}  & & \multirow{3}{*}{80.86} & 69.44 & \textbf{11.42}    \\
                        & EMinF                    &                        & 60.33 & \textbf{15.67} &                                  &                        & 64.19 & \textbf{16.67}  \\
                        & SubInj                   &                        & 37.00 & \textbf{39.00} &                                  &                        & 44.44 & \textbf{36.42} \\ 
\hline
\multirow{3}{*}{GAT}    & EMinS                    & \multirow{3}{*}{76.33} & 72.33 & 4.00           &  & \multirow{3}{*}{76.54} & 57.58 & \textbf{18.96}  \\
                        & EMinF                    &                        & 71.67 & \textbf{4.66}  &                                  &                        & 62.53 & \textbf{14.01}  \\
                        & SubInj                   &                        & 37.00 & \textbf{39.33} &                                  &                        & 44.13 & \textbf{32.14} \\ 
\hline
\multirow{3}{*}{GIN}    & EMinS                    & \multirow{3}{*}{71.67} & 41.67 & \textbf{30.00} & & \multirow{3}{*}{72.84} & 61.16 & \textbf{11.68} & \multirow{3}{*}{71.60} & 62.93 & 8.67   \\
                        & EMinF                    &                        & 41.67 & \textbf{30.00} &                                  &                        & 61.60 & \textbf{11.24} \\
                        & SubInj                   &                        & 36.67 & \textbf{35.00} &                                  &                        & 54.19 & \textbf{19.65} \\ 
\hline
\multirow{3}{*}{Sage}   & EMinS                    & \multirow{3}{*}{79.33} & 56.67 & \textbf{22.66} & \multirow{3}{*}{75.93} & 63.89 & \textbf{12.14} \\
                        & EMinF                    &                        & 65.33 & \textbf{14.00} &                                  &                        & 64.13 & \textbf{11.80} \\
                        & SubInj                   &                        & 40.33 & \textbf{39.00} &                                  &                        & 55.86 & \textbf{20.07}   \\
\bottomrule
\end{tabular}
}

\end{table*}


==> table/rebuttal/budget-EminF.tex <==
\begin{table*}
\centering
\caption{The effect of perturbation budget on the data protection performance and stealthiness of cloaked graph in terms of anomaly detection score. The results of applying error-minimizing-based methods EMinS and EMaxS on GCN are presented. }
\label{}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccccc} 
\toprule
\multirow{2}{*}{$\alpha$} & \multicolumn{2}{c}{MUTAG} & \multicolumn{2}{c}{ENZYMES} & \multicolumn{2}{c}{PROTEINS} & \multicolumn{2}{c}{IMDB-BINARY} & \multicolumn{2}{c}{IMDB-MULTI}  \\ 
\cline{2-11}
                          & Acc. $\downarrow$ & Dect. Score $\downarrow$   & Acc. $\downarrow$ & Dect. Score $\downarrow$     & Acc. $\downarrow$ & Dect. Score $\downarrow$      & Acc. $\downarrow$ & Dect. Score $\downarrow$         & Acc. $\downarrow$ & Dect. Score $\downarrow$                \\ 
\hline
0                         &           &               &           &                 &           &                  &           &                     &           &                            \\
0.005                      &           &               &           &                 &           &                  &           &                     &           &                            \\
0.010                       &           &               &           &                 &           &                  &           &                     &           &                            \\
0.015                         &           &               &           &                 &           &                  &           &                     &           &                            \\
0.020                       &           &               &           &                 &           &                  &           &                     &           &                            \\
0.025                       &           &               &           &                 &           &                  &           &                     &           &                            \\
0.030                      &           &               &           &                 &           &                  &           &                     &           &                            \\
\bottomrule
\end{tabular}

}

\end{table*}

==> table/rebuttal/budget-em.tex <==
\begin{table*}
\centering
\caption{The effect of perturbation budget on the data protection performance and stealthiness of cloaked graph in terms of anomaly detection score. The results of applying error-minimizing-based methods EMinS and EMaxS on GCN are presented. }
\label{}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccccccc} 
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{$\beta$} & \multicolumn{2}{c}{MUTAG} & \multicolumn{2}{c}{ENZYMES} & \multicolumn{2}{c}{PROTEINS} & \multicolumn{2}{c}{IMDB-BINARY} & \multicolumn{2}{c}{IMDB-MULTI}  \\ 
\cline{3-12}
                         &                          &Acc. $\downarrow$ & Dect. Score $\downarrow$   &Acc. $\downarrow$ & Dect. Score $\downarrow$     &Acc. $\downarrow$ & Dect. Score $\downarrow$      &Acc. $\downarrow$ & Dect. Score $\downarrow$         &Acc. $\downarrow$ & Dect. Score $\downarrow$                \\ 
\hline
\multirow{7}{*}{EMinS}   & 0                        &           &               &           &                 &           &                  &           &                     &           &                            \\
                         & 0.05                     &           &               &           &                 &           &                  &           &                     &           &                            \\
                         & 0.5                      &           &               &           &                 &           &                  &           &                     &           &                            \\
                         & 5                        &           &               &           &                 &           &                  &           &                     &           &                            \\
                         & 50                       &           &               &           &                 &           &                  &           &                     &           &                            \\
                         & 500                      &           &               &           &                 &           &                  &           &                     &           &                            \\
                         & 5000                     &           &               &           &                 &           &                  &           &                     &           &                            \\ 
\hline
\multirow{7}{*}{EMaxS}   & 0                        &           &               &           &                 &           &                  &           &                     &           &                            \\
                         & 0.05                     &           &               &           &                 &           &                  &           &                     &           &                            \\
                         & 0.5                      &           &               &           &                 &           &                  &           &                     &           &                            \\
                         & 5                        &           &               &           &                 &           &                  &           &                     &           &                            \\
                         & 50                       &           &               &           &                 &           &                  &           &                     &           &                            \\
                         & 500                      &           &               &           &                 &           &                  &           &                     &           &                            \\
                         & 5000                     &           &               &           &                 &           &                  &           &                     &           &                            \\
\bottomrule
\end{tabular}

}

\end{table*}

==> table/rebuttal/budget-subinj-n.tex <==
\begin{table*}
\centering
\caption{The effect of perturbation budget on the data protection performance and stealthiness of cloaked graph in terms of anomaly detection score. The results of applying error-minimizing-based methods EMinS and EMaxS on GCN are presented. }
\label{}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccccc} 
\toprule
\multirow{2}{*}{$n$} & \multicolumn{2}{c}{MUTAG}                    & \multicolumn{2}{c}{ENZYMES}                  & \multicolumn{2}{c}{PROTEINS}                 & \multicolumn{2}{c}{IMDB-BINARY}              & \multicolumn{2}{c}{IMDB-MULTI}         \\ 
\cline{2-11}
                     & Acc. $\downarrow$ & Dect. Score $\downarrow$ & Acc. $\downarrow$ & Dect. Score $\downarrow$ & Acc. $\downarrow$ & Dect. Score $\downarrow$ & Acc. $\downarrow$ & Dect. Score $\downarrow$ & Acc. $\downarrow$ & Dect. Score $\downarrow$  \\ 
\hline
3                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
4                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
5                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
6                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
7                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
8                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
9                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
\bottomrule
\end{tabular}


}

\end{table*}

==> table/rebuttal/budget-subinj-p.tex <==
\begin{table*}
\centering
\caption{The effect of perturbation budget on the data protection performance and stealthiness of cloaked graph in terms of anomaly detection score. The results of applying error-minimizing-based methods EMinS and EMaxS on GCN are presented. }
\label{}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccccc} 
\toprule
\multirow{2}{*}{$p$} & \multicolumn{2}{c}{MUTAG}                    & \multicolumn{2}{c}{ENZYMES}                  & \multicolumn{2}{c}{PROTEINS}                 & \multicolumn{2}{c}{IMDB-BINARY}              & \multicolumn{2}{c}{IMDB-MULTI}         \\ 
\cline{2-11}
                     & Acc. $\downarrow$ & Dect. Score $\downarrow$ & Acc. $\downarrow$ & Dect. Score $\downarrow$ & Acc. $\downarrow$ & Dect. Score $\downarrow$ & Acc. $\downarrow$ & Dect. Score $\downarrow$ & Acc. $\downarrow$ & Dect. Score $\downarrow$  \\ 
\hline
0.1                   &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
0.2                  &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
0.3                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
0.4                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
0.5                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
0.6                   &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
0.7                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
0.8                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
0.9                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
1.0                    &                   &                          &                   &                          &                   &                          &                   &                          &                   &                           \\
\bottomrule
\end{tabular}


}

\end{table*}

==> table/threat-exp-main.tex <==
\begin{table}[!thbp]
\caption{Comparison under different defense settings. }
\label{tab. compT}
    \label{c}
    \centering
\renewcommand{\arraystretch}{0.8}
\resizebox{0.7\linewidth}{!}{
% \begin{tabular}{ccccccccc} 
% \toprule
% \multirow{2}{*}{Methods} & \multirow{2}{*}{White-box} & \multicolumn{6}{c}{Grey-box}                                                                       & \multirow{2}{*}{Black-box}  \\ 
% \cmidrule{3-8}
%                          &                            & g1             & g2             & g3             & g4             & g5            & g6             &                             \\ 
% \midrule
% Clean                    & 50.20                      & 50.20          & 50.20          & 50.20          & 50.20          & 50.20         & 50.20          & 50.20                       \\
% Random                   & 49.33                      & 49.33          & 49.33          & 49.33          & 49.33          & 49.33         & 49.33          & 49.33                       \\
% EMaxS                    & 43.83                      & 45.5           & 42.5           & 43.67          & 44.17          & 50.83         & 47.33          & 50.5                        \\
% EMinS                    & \textbf{38.17}             & 46.17          & 41.83          & 40.0           & 49.17          & 46.17         & 47.0           & 47.83                       \\
% EMinF                    & 46.0                       & 46.83          & 41.67          & 48.83          & 44.17          & \textbf{38.0} & 40.5           & 47.83                       \\
% SubInj                   & 38.67                      & \textbf{38.67} & \textbf{38.67} & \textbf{38.67} & \textbf{38.67} & 38.67         & \textbf{38.67} & \textbf{38.67}              \\
% \bottomrule
% \end{tabular}
\begin{tabular}{ccccc} 
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{White-box} & \multicolumn{2}{c}{Grey-box}   & \multirow{2}{*}{Black-box}  \\ 
\cmidrule{3-4}
                         &                            & g1($\Acal$)           & g2($\Mcal$)             &                             \\ 
\midrule
Clean                    & 50.20                      & 50.20         & 50.20          & 50.20                       \\
Random                   & 49.33                      & 49.33         & 49.33          & 49.33                       \\
EMaxS                    & 43.83                      & 50.83         & 47.33          & 50.5                        \\
EMinS                    & \textbf{38.17}             & 46.17         & 47.0           & 47.83                       \\
EMinF                    & 46.0                       & \textbf{38.0} & 40.5           & 47.83                       \\
SubInj                   & 38.67                      & 38.67         & \textbf{38.67} & \textbf{38.67}              \\
\bottomrule
\end{tabular}
}

\end{table}


==> table/threat-exps-full.tex <==
\begin{table}[!thbp]
    \centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccccc} 
\toprule
\multirow{2}{*}{Datasets} & \multirow{2}{*}{Methods} & \multirow{2}{*}{White-box} & \multicolumn{6}{c}{Grey-box} & \multirow{2}{*}{Black-box}  \\ 
\cmidrule{4-9}
                          &                          &                            & g1 & g2 & g3 & g4 & g5 & g6  &                             \\ 
\midrule
\multirow{6}{*}{MUTAG}    & Clean                    & \multicolumn{8}{c}{}                                                                    \\
                          & Random                   & \multicolumn{8}{c}{}                                                                    \\
                          & EMaxS                    &                            &    &    &    &    &    &     &                             \\
                          & EMinS                    &                            &    &    &    &    &    &     &                             \\
                          & EMinF                    &                            &    &    &    &    &    &     &                             \\
                          & SubInj                   & \multicolumn{8}{c}{}                                                                    \\
                          \midrule
\multirow{6}{*}{IMDB-MULTI}    & Clean                    & \multicolumn{8}{c}{}                                                                    \\
                          & Random                   & \multicolumn{8}{c}{}                                                                    \\
                          & EMaxS                    &                            &    &    &    &    &    &     &                             \\
                          & EMinS                    &                            &    &    &    &    &    &     &                             \\
                          & EMinF                    &                            &    &    &    &    &    &     &                             \\
                          & SubInj                   & \multicolumn{8}{c}{}                                                                    \\
\bottomrule
\end{tabular}
}
    \caption{Performance comparison under different defense settings. }
    \label{tab:thread-mdoel-exp}
\end{table}


==> table/time-table-detailed.tex <==
\begin{table}[htbp]
\caption{The time for training noise generator on six different datasets with a GCN source model. 
% \rtodo{fill all the cases}
}
\label{tab:gen-time}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccccccc}
\toprule
     Datasets   & Random & EMaxS      & EMinS      & EMinF    & SubInj  \\
\midrule
MUTAG   & 29s    & 23h31m24s  & 23h21m26s  & 3h13m42s & 46s     \\
ENZYMES & 1m47s  & 78h45m22s  & 82h50m20s  & 4h49m47s & 2m17s   \\
PROTEINS& 2m10s  & 5h32m3s    & 6h4m57s    & 29m33s   & 38s     \\
IMDB-BINARY & 2m11s & 6h30m7s & 6h59m3s  & 2h14m8s  & 1m2s     \\
IMDB-MULTI  & 3m15s & 21h27m23s & 19h42m4s & 4h12m53s & 7m53s    \\
COLLAB  & 13m4s  & 64h48m29s  & 164h47m52s & 3h9m11s  & 25m     \\
\bottomrule
\end{tabular}
}

\end{table}
